Mesh Strikes Back: Fast and Efficient Human Reconstruction from RGB videos

Human reconstruction and synthesis from monocular RGB videos is a challenging problem due to clothing, occlusion, texture discontinuities and sharpness, and framespecific pose changes. Many methods employ deferred rendering, NeRFs and implicit methods to represent clothed humans, on the premise that mesh-based representations cannot capture complex clothing and textures from RGB, silhouettes, and keypoints alone. We provide a counter viewpoint to this fundamental premise by optimizing a SMPL+D mesh and an efficient, multi-resolution texture representation using only RGB images, binary silhouettes and sparse 2D keypoints. Experimental results demonstrate that our approach is more capable of capturing geometric details compared to visual hull, mesh-based methods. We show competitive novel view synthesis and improvements in novel pose synthesis compared to NeRF-based methods, which introduce noticeable, unwanted artifacts. By restricting the solution space to the SMPL+D model combined with differentiable rendering, we obtain dramatic speedups in compute, training times (up to 24x) and inference times (up to 192x). Our method therefore can be used as is or as a fast initialization to NeRF-based methods.

==> sections/notes.tex <==
\section{Notes (Remove Later)}
\label{sec:notes}

\brandon{Note.}

\rohit{Note.}

\sid{Note.}

\ganesh{Note.}


\subsection{Literature}

\subsubsection{Avatar Generation}
People Snapshot~\cite{alldieck:cvpr2018:peoplesnap}

Detailed Human Avatars from Monocular Video~\cite{alldieck:3dv2018:humanmono}

Neural Body~\cite{peng:cvpr2021:neuralbod}

Anim-NeRF~\cite{chen:arxiv2021:animner}

Synthetic data looks very much like “cartoons” -- basically the uncanny valley problem in synthetic human generation.~\cite{wang:cvpr2022:clonedperson}

PINA uses depth sensors to generate personalized and animatable neural avatars from RGB-D videos.~\cite{dong:cvpr2022:pina}

Capturing and Animation of Body and Clothing from Monocular Video. Model the body with SMPL-X, model clothing with NeRF.~\cite{yao:arxiv2022:monoclothedbody}

Animatable Volume Rendering of Articulated Human SDFs~\cite{wang:eccv2022:arah}

\subsubsection{Face Verification}

Cosine sim for face verification~\cite{hieu:accv2010:cosface}

Face verification~\cite{cao:cvpr2018:facerec}
